Confident Multiple Choice Learning

Ensemble methods are arguably the most trustworthy techniques for boosting the performance of machine learning models. Popular independent ensembles (IE) relying on naive averaging/voting scheme have been of typical choice for most applications involving deep neural networks, but they do not consider advanced collaboration among ensemble models. In this paper, we propose new ensemble methods specialized for deep neural networks, called confident multiple choice learning (CMCL): it is a variant of multiple choice learning (MCL) via addressing its overconfidence issue.In particular, the proposed major components of CMCL beyond the original MCL scheme are (i) new loss, i.e., confident oracle loss, (ii) new architecture, i.e., feature sharing and (iii) new training method, i.e., stochastic labeling. We demonstrate the effect of CMCL via experiments on the image classification on CIFAR and SVHN, and the foreground-background segmentation on the iCoseg. In particular, CMCL using 5 residual networks provides 14.05% and 6.60% relative reductions in the top-1 error rates from the corresponding IE scheme for the classification task on CIFAR and SVHN, respectively.

==> backup.tex <==
\begin{table*}[]
\centering
\begin{tabular}{cccllll}
\hline
\multirow{2}{*}{Model Name}               &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ensemble\\Method\end{tabular}} &
\multicolumn{2}{l}{\hspace{18mm}CIFAR-10} &
\multicolumn{2}{l}{\hspace{22mm}SVHN} \\
& &
Oracle Error Rate  &
Top-1 Error Rate &
Oracle Error Rate  &
Top-1 Error Rate   \\ \hline
\multirow{4}{*}{VGGNet-17}    & - (single)           & \hspace{0mm}10.65\%                    &\hspace{6mm}10.65\%    & \hspace{8mm}5.22\%                    & \hspace{7mm}5.22\%       \\
& IE           & \hspace{0mm}3.27\%                    & \hspace{7mm}8.21\%    & \hspace{8mm}1.99\%                    & \hspace{7mm}4.10\%       \\
                           & MCL          & \hspace{0mm}\textbf{2.52\%}                    & \hspace{6mm}45.58\%    & \hspace{8mm}\textbf{1.45\%}                    & \hspace{6mm}45.30\%         \\
                           & CMCL         & \hspace{0mm}2.95\% & \hspace{7mm}\textbf{7.83\% (-4.63\%)}  & \hspace{8mm}1.65\% & \hspace{7mm}\textbf{3.92\% (-4.39\%)} \\ \hline
\multirow{4}{*}{GoogLeNet-18} & - (single)           & \hspace{0mm}10.15\%                    & \hspace{6mm}10.15\%    & \hspace{8mm}4.59\%                    & \hspace{7mm}4.59\%       \\
& IE           & \hspace{0mm}3.37\%                    & \hspace{7mm}7.97\%    & \hspace{8mm}1.78\%                    & \hspace{7mm}3.60\%       \\
                           & MCL          & \hspace{0mm}\textbf{2.41\%}           & \hspace{6mm}52.03\% & \hspace{8mm}1.39\%           & \hspace{6mm}37.92\%         \\
                           & CMCL         & \hspace{0mm}2.54\%                    & \hspace{7mm}\textbf{7.44\% (-6.65\%)}
                           &\hspace{8mm}\textbf{1.31\%}                    & \hspace{7mm}\textbf{3.46\% (-3.89\%)}  \\ \hline
\multirow{4}{*}{ResNet-32} & - (single)           & 12.89\%                    & \hspace{6mm}12.89\%    & \hspace{8mm}5.05\%                    & \hspace{7mm}5.05\%       \\
& IE           & \hspace{0mm}3.54\%                    & \hspace{7mm}9.50\% & \hspace{8mm}1.81\%                    & \hspace{7mm}3.84\%         \\
                           & MCL          & \hspace{0mm}3.11\%           & \hspace{6mm}53.74\% & \hspace{8mm}1.69\%           & \hspace{6mm}39.76\%         \\
                           & CMCL         & \hspace{0mm}\textbf{2.89\%}                    & \hspace{7mm}\textbf{8.42\% (-11.37\%)}
                           & \hspace{8mm}\textbf{1.41\%}                    & \hspace{7mm}\textbf{3.56\% (-7.29\%)}\\ \hline
\end{tabular}
\caption{Classification test set error rates on CIFAR-10 and SVHN for various large-scale CNN models. 
\textcolor{blue}{We train an ensemble of 5 models, and use CMCL with both feature sharing and stochastic labeling.}
Boldface values in parentheses indicate relative error rate reductions from the best results of MCL and IE.}
\label{tbl:deep}
\end{table*}

\begin{itemize}
\item[(a)] First, generate a set of plausible outputs.
\item[(b)] Then, pick the correct solution from the set.
\end{itemize}
{\bf Organization.}
In Section \ref{sec:relatedwork}, we introduce necessary backgrounds for multiple choice learning
and the corresponding loss function.
We describe the proposed loss and the corresponding training scheme in Section \ref{sec:model}.
Section \ref{sec:feature-gen} provides additional techniques for the proposed ensemble model.
Experimental results are reported in Section \ref{sec:exp}.
\iffalse
For 
we first verify that we can generate a set of diverse/plausible confidential predictions by optimizing {\em confidential oracle loss} using {\em CMCL}.
When we train ensemble of 5 CNNs with 2 convolutional layers, 
we can achieve up to 66.88 \% relative reduction in top-1 classification error using {\em CMCL} \textcolor{blue}{against original {\em MCL} \cite{mcl16}}
while keeping similar \textcolor{blue}{specialization effects}.
In addition, using {\em CMCL} with {\em stochastic feature sharing} and {\em stochastic labeling}, we can outperform all baselines (i.e., independent ensemble and \textcolor{blue}{original} {\em MCL}) with respect to both oracle and top-1 error by extracting the general features and improving the generalization effects.
In particular, ensemble of 5 residual networks \cite{resnet} trained by {\em CMCL} achieve the 15\% and 83\% relative reductions in top-1 classification against independent ensemble and \textcolor{blue}{original} {\em MCL}, respectively.
Throughout these experiments, we verify the efficacy of {\em CMCL} using various CNNs which have shown the state-of-art performances on image classification. 
We also demonstrate the broad applicability of {\em CMCL} for background-foreground segmentation task on iCoseg dataset \cite{icoseg10}.
The ensemble of 2 FCNs trained by {\em CMCL} generates high quality solutions by specializing to specific images while that of 2 FCNs trained by independent ensemble do not.
Also, {\em CMCL} improves both oracle and top-1 error compared to all baselines for this task.
\fi
%We propose both a general iterative algorithm for optimizing the suggested objective function, and scalable one based on stochastic gradient descent methods.

\iffalse
Although there have been several efforts to apply various ensemble methods such as bagging and boosting to deep models \cite{zhou2002ensembling, carney1999tuning}, it is well-known that traditional/naive ensembles which independently train models with random initialization have achieved the best performance in general \cite{ciregan2012multi,lee2015m}.
In contrast with this conjecture, we show that confident {\em MCL} corresponding to bagging-like ensemble method can also improve the performance over traditional ensembles.
In addition, we present advanced techniques specialized for deep models such as feature sharing and Monte Carlo estimator of gradients. 
Using these methods, we demonstrate the broad applicability and efficacy of {\em CMCL} on a wide range of problem domains such as image classification and segmentation.
\fi


\iffalse
Ensembles of deep neural networks such as convolutional network networks (CNNs) and recurrent neural networks (RNNs)
have demonstrated state-of-the-art performance on many high-profile competitions such as the ILSVRC challenge \citep{imagenet12} and Kaggle competitions.
The traditional ensembles, which train several models independently and combine them with majority voting or averaging \cite{caruana2004ensemble}, generally improve the performance by utilizing model variation induced by bagging or random initialization.
\fi

% problem of specialization - (1) uncertainty and (2) saying only trained answer

% our propsoed method

% organization
\iffalse
{\bf Organization.}
Section \ref{sec:relatedwork} provides some preliminaries.
In Section \ref{sec:model}, we present a new objective and training algorithm for optimizing it.
Section \ref{sec:feature-gen} provides advanced techniques, specialized for deep models for improving the performance.
In Section \ref{sec:exp}, 
we show performances of our algorithm through extensive experiments.
\fi



\iffalse
In this section, we propose more scalable training algorithm based on the above algorithm.
Although the stochastic algorithm proposed in Section \ref{sec:alg} relaxes the complexity issues, 
it still might suffer from a complexity issue since we also consider the entropy in our optimization problem \eqref{eq:objective}.
One can note that
computing the entropy and gradient of it can be \textcolor{blue}{intractable} for large numbers of classes, \textcolor{blue}{e.g., 1000 for ILSVRC challenge \cite{imagenet12}}, since it requires summations over all possible configurations of classes.
To handle this issue, we first simplify the assignment of flag variables in \eqref{eq:assignflag} such that
assigning the flag variables using the training loss $\ell \left( y,P_{\theta}\left(y \mid \mathbf{x} \right) \right)$, i.e., ignoring the entropy term.
This heuristic might be reasonably work well since the training loss can be dominant compared to entropy term. 
For example, in case of the cross entropy loss which is the most popular training loss in machine learning field,
this assumption can be mild since the cross entropy is unbounded while the entropy is not.
By ignoring the entropy term, we can significantly reduce the complexity of algorithm (i.e., we can reduce the complexity of $O\left( | \mathcal{Y}| \right)$ in the assignment step).
Also, for the same reason, computing the gradient of entropy can be also \textcolor{blue}{intractable}.
We handle this issue by proposing a simple stochastic method for estimating the gradient of entropy using Monte Carlo approximation.
We first note that maximizing the entropy of the predictive distribution is equivalent 
to making it be closer to uniform distribution.
Therefore, we consider minimizing the KL divergence from the predictive distribution to uniform distribution as follows: 
\begin{align*}
& KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) \\
& = \sum \limits_y Q \left( y \right) \log \frac{Q \left( y \right)}{P_{\theta}\left( y\mid \mathbf{x} \right)} \\
&= \sum \limits_y Q \left( y \right) \log Q \left( y \right) - \sum \limits_y Q \left( y \right) {P_{\theta}\left( y\mid \mathbf{x} \right)},
\end{align*}
where $Q \left( y \right)$ is uniform distribution.
One can note that the gradient of $ KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right)$ with respect to the model parameter $\theta$ becomes 
\begin{align*}
 \bigtriangledown_{\theta} KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) & = - \sum \limits_y Q \left( y \right)  \bigtriangledown_{\theta} {P_{\theta}\left( y\mid \mathbf{x} \right)} \\
& = - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {\log P_{\theta}\left( y\mid \mathbf{x} \right)} ].
\end{align*}
For estimating this expectation, we use the following Monte Carlo approximation:
\begin{align*}
& - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {\log P_{\theta}\left( y\mid \mathbf{x} \right)} ]
\backsimeq - \frac{1}{S} \sum_s \bigtriangledown_{\theta} {\log P_{\theta}\left( y^{s}\mid \mathbf{x} \right)},
\end{align*}
where $y^{s} \sim Q \left( y \right)$ and $S$ is the number of samples.
This random estimator takes samples from the uniform distribution $Q \left( y \right)$ 
and constructs estimates of the gradient using them.
It is well-known that the resulting estimator is unbiased and has relatively low variance \cite{sfnn13}.
We remark that this corresponds to the gradient of the cross entropy loss using a random class which is sampled from uniform distribution for $S=1$.
\fi



\iffalse
inspired by \cite{mcl16}, we replace the iterative assignment of flag variables with batch updates in stochastic gradient descent.
Instead of alternating between assigning flag variables and re-training every model, 
we assign flag variables and update model parameters using back-propagation once per random batch.
\textcolor{blue}{Here, we note that we simplify the Step 1 by assigning the flag variables using the cross entropy loss.
Since the cross entropy is unbounded while the entropy is not, 
we think that it is dominant in optimizing the objective.
By ignoring the entropy term, we can significantly reduce the complexity of algorithm.}
\fi

%In our experiments,  using a simple averaging method.



\iffalse
\textcolor{blue}{In this section, we separately describe our algorithm for minimizing the objective function \eqref{eq:objective}.}
%We describe our algorithm based on stochastic gradient descent and Monte Carlo approximation
The parameters of ensemble models can be learned using a variant of the backpropagation algorithm \cite{backprop85}.
However, one can note that directly optimizing our objective function \eqref{eq:objective} is not trivial 
since there are two issues: optimizing the $\min$ function and computing the gradient of the entropy constraint.
First, consider the first term of \eqref{eq:objective}, i.e., 
\begin{align}
\sum \limits_{i=1}^N  \bigg( \min \limits_{m\in [M]} \ell \left( y_i, P_{\theta_m} \left( y = y_i \mid \mathbf{x}_i \right) \right) \bigg).
\label{eq:firstterm}
\end{align}
Directly minimizing this term is difficult since the $\min$ function is non-continuous and non-convex function.
%As mentioned in Section \ref{sec:uncer},
In order to handle this issue,
\citep{mcl12} present an objective which replaces the $\min$ in the loss with flag variables $\left( p_i^m \right)_{m=1}^M$ which is 1 if learner $m$ produces the smallest error on input $\mathbf{x}_i$ as follows:
\begin{align}
\label{eq:relaxed}
&\underset{p_i^m, \theta_m }{\arg \min} \quad \sum \limits_{i=1}^N \sum \limits_{m=1}^M p_i^m \ell \left( y_i, P_{\theta_m} \left( y = y_i \mid \mathbf{x}_i \right) \right) \\
& \quad\text{subject to} \quad \sum_{m=1}^M p_i^m = 1, \quad \forall i. \nonumber
\end{align}
Optimizing this joint problem \eqref{eq:relaxed} corresponds to 
minimizing the (potentially tight) upper-bound of the first term \eqref{eq:firstterm} \cite{mcl12}.
Recently, \citep{mcl16} proposed a stochastic gradient descent based algorithm.
For each random batch, 
it first computes losses from each ensemble member.
Then, during the backward pass, 
the gradient of the loss for each data is backpropagated only to the lowest error model on that data.
We use this simple and efficient algorithm for optimizing the first term of \eqref{eq:objective}.
\fi

\iffalse
\textcolor{blue}{
Next, consider the second term of \eqref{eq:objective}, i.e., 
\begin{align*}
\label{eq:second}
  \sum \limits_{i=1}^N    \sum \limits_{{\widehat m} \in [M] \backslash \{ m \} } \sum \limits_{y} P_{\theta_{{\widehat m}}}\left( y \mid \mathbf{x}_i  \right) \log P_{\theta_{{\widehat m}}}\left(y \mid \mathbf{x}_i \right).
\end{align*}}
Although we can optimize this term using a variant of the backpropagation algorithm \cite{backprop85},
computing gradients of the entropy constraint can be intractable 
for large numbers of classes, \textcolor{blue}{e.g., 1000 for ILSVRC challenge \cite{imagenet12}}, since it requires summations over all possible configurations of classes.
In order to handle this issue, we propose a simple stochastic method using Monte Carlo approximation.
We first note that maximizing the entropy of the predictive distribution is equivalent 
to making it be closer to uniform distribution.
Therefore, we consider minimizing the KL divergence from the predictive distribution to uniform distribution as follows: 
\begin{align*}
& KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) \\
& = \sum \limits_y Q \left( y \right) \log \frac{Q \left( y \right)}{P_{\theta}\left( y\mid \mathbf{x} \right)} \\
&= \sum \limits_y Q \left( y \right) \log Q \left( y \right) - \sum \limits_y Q \left( y \right) {\log P_{\theta}\left( y\mid \mathbf{x} \right)},
\end{align*}
where $Q \left( y \right)$ is uniform distribution.
One can note that the gradient of $ KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right)$ with respect to the model parameter $\theta$ becomes 
\begin{align*}
 \bigtriangledown_{\theta} KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) & = - \sum \limits_y Q \left( y \right)  \bigtriangledown_{\theta} {P_{\theta}\left( y\mid \mathbf{x} \right)} \\
& = - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {P_{\theta}\left( y\mid \mathbf{x} \right)} ].
\end{align*}
For estimating this expectation, we use the following Monte Carlo approximation:
\begin{align*}
& - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {P_{\theta}\left( y\mid \mathbf{x} \right)} ]
\backsimeq - \frac{1}{S} \sum_s \bigtriangledown_{\theta} {P_{\theta}\left( y^{s}\mid \mathbf{x} \right)},
\end{align*}
where $y^{s} \sim Q \left( y \right)$ and $S$ is the number of samples.
This random estimator takes samples from the uniform distribution $Q \left( y \right)$ 
and constructs estimates of the gradient using them.
It is well-known that the resulting estimator is unbiased and has relatively low variance \cite{sfnn13}.
We remark that this corresponds to the gradient of the cross entropy loss using a random class which is sampled from uniform distribution for $S=1$.
\fi

\iffalse
Using these two ideas, we propose a straightforward optimization algorithm for optimization problem \eqref{eq:objective} 
based on stochastic gradient descent as shown in Algorithm \ref{alg:our}.
For each random batch, we calculate losses from each ensemble member by passing the data through them. 
Then, during the backward pass, 
the gradient of the loss for each data is backpropagated only to the lowest error model on that data, and the gradient of the cross entropy loss computed by random class is backpropagated to remaining models. 
\textcolor{blue}{
We remark that this algorithm has same time-complexity compared to sMCL algorithm proposed by \cite{mcl16}.
Experimental results.
}
\fi



\iffalse
We also provide a simple gradient estimator of entropy loss for reducing the training time.
One can note that computing the gradient of the entropy loss $H$ can be \textcolor{blue}{time-consuming task} for large numbers of classes, \textcolor{blue}{e.g., 1000 for ILSVRC challenge \cite{imagenet12}}, since it requires summations over all possible configurations of classes.
We handle this issue by proposing a simple stochastic method for estimating the gradient of entropy using Monte Carlo approximation.
We first note that maximizing the entropy of the predictive distribution is equivalent 
to making it be closer to uniform distribution.
Therefore, we consider minimizing the KL divergence from the predictive distribution to uniform distribution as follows: 
\begin{align*}
& KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) \\
& = \sum \limits_y Q \left( y \right) \log \frac{Q \left( y \right)}{P_{\theta}\left( y\mid \mathbf{x} \right)} \\
&= \sum \limits_y Q \left( y \right) \log Q \left( y \right) - \sum \limits_y Q \left( y \right) {\log P_{\theta}\left( y\mid \mathbf{x} \right)},
\end{align*}
where $Q \left( y \right)$ is uniform distribution.
One can note that the gradient of $ KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right)$ with respect to the model parameter $\theta$ becomes 
\begin{align*}
 \bigtriangledown_{\theta} KL \left( Q \left( y \right) \parallel P_{\theta}\left( y\mid \mathbf{x} \right) \right) & = - \sum \limits_y Q \left( y \right)  \bigtriangledown_{\theta} {\log P_{\theta}\left( y\mid \mathbf{x} \right)} \\
& = - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {\log P_{\theta}\left( y\mid \mathbf{x} \right)} ].
\end{align*}
For estimating this expectation, we use the following Monte Carlo approximation:
\begin{align*}
& - \E_{Q \left( y \right)} [ \bigtriangledown_{\theta} {\log P_{\theta}\left( y\mid \mathbf{x} \right)} ]
\backsimeq - \frac{1}{S} \sum_s \bigtriangledown_{\theta} {\log P_{\theta}\left( y^{s}\mid \mathbf{x} \right)},
\end{align*}
where $y^{s} \sim Q \left( y \right)$ and $S$ is the number of samples.
This random estimator takes samples from the uniform distribution $Q \left( y \right)$ 
and constructs estimates of the gradient using them.
It is well-known that the resulting estimator is unbiased and has relatively low variance \cite{sfnn13}.
We remark that this corresponds to the gradient of the cross entropy loss using a random class which is sampled from uniform distribution for $S=1$.
In summary, for each random batch, we calculate the training losses from each ensemble member by passing the data through them. 
Then, during the backward pass, 
the gradient of the loss computed by true class for each data is backpropagated only to the lowest error model on that data, and the gradient of the cross entropy loss computed by random class is backpropagated to remaining models. 
We call this algorithm as Confidential stochastic multiple choice learning (sMCL), as shown in Algorithm \ref{alg:our}.
\fi

\iffalse
replacing the iterative assignment of flag variables with batch updates in stochastic gradient descent.
Instead of alternating between assigning flag variables and re-training every model, 
we assign flag variables according to \eqref{eq:assignflag} and update model parameters using back-propagation once per random batch.
\textcolor{blue}{One can note that this stochastic algorithm significantly can save time since ensemble models need only be trained to convergence once in parallel.}
\fi


\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{@{}ccccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Overlap Parameter $K$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=5$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=10$ \end{tabular}} \\ &
                                \multicolumn{1}{c}{} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} & &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} \\ \midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 1 \end{tabular}} &
    \multicolumn{1}{c}{69.70 $\%$} &
    \multicolumn{1}{c}{42.37 $\%$} &
    \multicolumn{1}{c}{74.05 $\%$} &
    \multicolumn{1}{c}{29.48 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{68.07 $\%$} &
    \multicolumn{1}{c}{52.40 $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 2 \end{tabular}} &
    \multicolumn{1}{c}{72.53 $\%$} &
    \multicolumn{1}{c}{52.19 $\%$} &
    \multicolumn{1}{c}{79.29 $\%$} &
    \multicolumn{1}{c}{46.04 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL 
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{70.85 $\%$} &
    \multicolumn{1}{c}{55.23 $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 3 \end{tabular}} &
    \multicolumn{1}{c}{72.33 $\%$} &
    \multicolumn{1}{c}{54.90 $\%$} &
    \multicolumn{1}{c}{79.15 $\%$} &
    \multicolumn{1}{c}{50.80 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{71.26 $\%$} &
    \multicolumn{1}{c}{56.34 $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 4 \end{tabular}} &
    \multicolumn{1}{c}{70.86 $\%$} &
    \multicolumn{1}{c}{56.46 $\%$} &
    \multicolumn{1}{c}{78.57 $\%$} &
    \multicolumn{1}{c}{53.28 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{70.36 $\%$} &
    \multicolumn{1}{c}{56.79 $\%$} &
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{ $\%$} &
    \multicolumn{1}{c}{ $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Classification test set accuracy on CIFAR-10.
}\label{tbl:cifar10}
\end{table*}


\iffalse
\begin{figure} [t] \centering
\includegraphics [width=0.5\textwidth]{./figures/ensemble_acc.eps}
\,
\caption{Test set accuracy comparison for varying the ensemble size $M$.}
\label{fig:mclnn}
\end{figure}
\fi

\iffalse
\begin{table*}[h]
\begin{center}
\small
\begin{tabular}{@{}lcccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Overlap Parameter $K$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=5$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=10$ \end{tabular}} \\ &
                                \multicolumn{1}{c}{} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} & &
    \multicolumn{1}{c}{86.58 $\%$} &
    \multicolumn{1}{c}{81.29 $\%$} &
    \multicolumn{1}{c}{88.11 $\%$} &
    \multicolumn{1}{c}{81.27 $\%$} \\ \midrule
    
\begin{tabular}{c} sMCL     \end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 1 \end{tabular}} &
    \multicolumn{1}{c}{93.84 $\%$} &
    \multicolumn{1}{c}{38.67 $\%$} &
    \multicolumn{1}{c}{100.0 $\%$} &
    \multicolumn{1}{c}{25.47 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL            \end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{93.34 $\%$} &
    \multicolumn{1}{c}{80.04 $\%$} &
    \multicolumn{1}{c}{98.10 $\%$} &
    \multicolumn{1}{c}{78.85 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.7)  \end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{96.04 $\%$} &
    \multicolumn{1}{c}{84.67 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.9)    \end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{96.33 $\%$} &
    \multicolumn{1}{c}{84.91 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL     \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 2 \end{tabular}}  &
    \multicolumn{1}{c}{94.79 $\%$} &
    \multicolumn{1}{c}{72.19 $\%$} &
    \multicolumn{1}{c}{96.95 $\%$}&
    \multicolumn{1}{c}{49.68 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{95.07 $\%$}  &
    \multicolumn{1}{c}{82.38 $\%$} &
    \multicolumn{1}{c}{97.60 $\%$} &
    \multicolumn{1}{c}{80.44 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{96.07 $\%$} &
    \multicolumn{1}{c}{85.00 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{95.96 $\%$} &
    \multicolumn{1}{c}{85.17 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 3 \end{tabular}} & 
    \multicolumn{1}{c}{91.57 $\%$}  &
    \multicolumn{1}{c}{79.08 $\%$} &
    \multicolumn{1}{c}{98.13 $\%$}&
    \multicolumn{1}{c}{72.05 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{94.78 $\%$}  &
    \multicolumn{1}{c}{83.72 $\%$} &
    \multicolumn{1}{c}{98.19 $\%$} &
    \multicolumn{1}{c}{81.89 $\%$}\\  
\begin{tabular}{c} Confidential sMCL + FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{95.66 $\%$} &
    \multicolumn{1}{c}{85.31 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{95.23 $\%$} &
    \multicolumn{1}{c}{85.37 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 4 \end{tabular}}  & 
    \multicolumn{1}{c}{92.00 $\%$}  &
    \multicolumn{1}{c}{80.56 $\%$} &
    \multicolumn{1}{c}{96.49 $\%$}&
    \multicolumn{1}{c}{75.76 $\%$}  \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c} \end{tabular}  &
    \multicolumn{1}{c}{93.24 $\%$}  & 
    \multicolumn{1}{c}{83.90 $\%$} & 
    \multicolumn{1}{c}{97.84 $\%$} & 
    \multicolumn{1}{c}{82.48 $\%$} \\  
\begin{tabular}{c} Confidential sMCL + FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{94.23 $\%$} &
    \multicolumn{1}{c}{85.19 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL + FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  &
    \multicolumn{1}{c}{93.95 $\%$} &
    \multicolumn{1}{c}{85.36 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Classification test set accuracy on CIFAR-10 using light convNet.
}\label{tbl:loc}
\end{table*}
\fi

\iffalse
\begin{table*}[h]
\begin{center}
\small
\begin{tabular}{@{}lcccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Overlap Parameter $K$ \end{tabular}}
 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=5$ \end{tabular}} &  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=10$ \end{tabular}} \\ 
& \multicolumn{1}{c}{} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} & & \multicolumn{1}{c}{89.84 $\%$} & \multicolumn{1}{c}{85.26 $\%$} & \multicolumn{1}{c}{91.34 $\%$} & \multicolumn{1}{c}{85.35 $\%$} \\ \midrule
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 1 \end{tabular}}  & \multicolumn{1}{c}{95.71 $\%$}  & \multicolumn{1}{c}{47.26 $\%$} & \multicolumn{1}{c}{100 $\%$}& \multicolumn{1}{c}{22.41 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.61 $\%$} & \multicolumn{1}{c}{84.07 $\%$}  & \multicolumn{1}{c}{98.84 $\%$}& \multicolumn{1}{c}{84.28 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.52 $\%$} & \multicolumn{1}{c}{85.12 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.94 $\%$} & \multicolumn{1}{c}{85.32 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\\midrule
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 2 \end{tabular}}  & \multicolumn{1}{c}{96.15 $\%$}  & \multicolumn{1}{c}{78.40 $\%$} & \multicolumn{1}{c}{99.04 $\%$}& \multicolumn{1}{c}{57.03 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.48 $\%$}  & \multicolumn{1}{c}{85.21 $\%$} & \multicolumn{1}{c}{ $\%$} & \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.40 $\%$} & \multicolumn{1}{c}{85.60 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.31 $\%$} & \multicolumn{1}{c}{85.77 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\\midrule
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 3 \end{tabular}} & \multicolumn{1}{c}{95.39 $\%$}  & \multicolumn{1}{c}{83.87 $\%$} & \multicolumn{1}{c}{98.51 $\%$}& \multicolumn{1}{c}{78.76 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.54 $\%$}  & \multicolumn{1}{c}{85.57 $\%$} & \multicolumn{1}{c}{ $\%$} & \multicolumn{1}{c}{ $\%$}\\  
\begin{tabular}{c} Confidential sMCL+FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.58 $\%$} & \multicolumn{1}{c}{85.73 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.73 $\%$} & \multicolumn{1}{c}{85.70 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\\midrule
\begin{tabular}{c} sMCL  \end{tabular}& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 4 \end{tabular}}  & \multicolumn{1}{c}{94.27 $\%$}  & \multicolumn{1}{c}{84.98 $\%$} & \multicolumn{1}{c}{98.02 $\%$}& \multicolumn{1}{c}{82.19 $\%$}  \\ 
\begin{tabular}{c} Confidential sMCL  \end{tabular}& \begin{tabular}{c} \end{tabular}  & \multicolumn{1}{c}{94.18 $\%$}  & \multicolumn{1}{c}{ 85.25 $\%$} & \multicolumn{1}{c}{98.19 $\%$} & \multicolumn{1}{c}{85.65 $\%$} \\  
\begin{tabular}{c} Confidential sMCL+FS(0.7) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{94.06 $\%$} & \multicolumn{1}{c}{85.68 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\ 
\begin{tabular}{c} Confidential sMCL+FS(0.9) \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{93.86 $\%$} & \multicolumn{1}{c}{85.72 $\%$}  & \multicolumn{1}{c}{ $\%$}& \multicolumn{1}{c}{ $\%$} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Classification test set accuracy on CIFAR-10 using Lenet.
}\label{tbl:loc}
\end{table*}
\fi


\iffalse
\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{@{}lcccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Ensemble Size \end{tabular}}
 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} CIFAR-10 \end{tabular}} &  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} CIFAR-100 \end{tabular}} \\ 
& \multicolumn{1}{c}{} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} &\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}} 5 \end{tabular}} & \multicolumn{1}{c}{90.73 $\%$} & \multicolumn{1}{c}{85.21 $\%$} & \multicolumn{1}{c}{68.22 $\%$} & \multicolumn{1}{c}{53.33 $\%$} \\
\begin{tabular}{c} sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.09 $\%$}  & \multicolumn{1}{c}{96.09 $\%$} & \multicolumn{1}{c}{71.29 $\%$}& \multicolumn{1}{c}{42.81 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.19 $\%$} & \multicolumn{1}{c}{85.21 $\%$}  & \multicolumn{1}{c}{\textcolor{red}{63.26} $\%$}& \multicolumn{1}{c}{49.58 $\%$} \\ 
\begin{tabular}{c} sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{96.49 $\%$}  & \multicolumn{1}{c}{80.57 $\%$} & \multicolumn{1}{c}{72.69 $\%$}& \multicolumn{1}{c}{51.45 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.48 $\%$}  & \multicolumn{1}{c}{85.49 $\%$} & \multicolumn{1}{c}{\textcolor{red}{68.05} $\%$} & \multicolumn{1}{c}{52.09 $\%$} \\ 
\begin{tabular}{c} sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.00 $\%$}  & \multicolumn{1}{c}{83.81 $\%$} & \multicolumn{1}{c}{72.22 $\%$}& \multicolumn{1}{c}{\textcolor{red}{54.00} $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{94.71 $\%$}  & \multicolumn{1}{c}{85.56 $\%$} & \multicolumn{1}{c}{70.50 $\%$} & \multicolumn{1}{c}{53.82 $\%$}\\ 
\begin{tabular}{c} sMCL (top 4)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{93.00 $\%$}  & \multicolumn{1}{c}{84.87 $\%$} & \multicolumn{1}{c}{69.55 $\%$}& \multicolumn{1}{c}{\textcolor{red}{53.89} $\%$}  \\ 
\begin{tabular}{c} Confidential sMCL (top 4)  \end{tabular}& \begin{tabular}{c} \end{tabular}  & \multicolumn{1}{c}{94.41 $\%$}  & \multicolumn{1}{c}{85.70 $\%$} & \multicolumn{1}{c}{69.30 $\%$} & \multicolumn{1}{c}{53.96 $\%$} \\  
\midrule
\begin{tabular}{c} Independent \end{tabular} &\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}} 10 \end{tabular}} & \multicolumn{1}{c}{92.36 $\%$} & \multicolumn{1}{c}{85.20 $\%$}& \multicolumn{1}{c}{74.28 $\%$} & \multicolumn{1}{c}{54.35 $\%$} \\
\begin{tabular}{c} sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{100 $\%$}  & \multicolumn{1}{c}{20.82 $\%$} & \multicolumn{1}{c}{78.49 $\%$} & \multicolumn{1}{c}{35.72 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{97.90 $\%$}  & \multicolumn{1}{c}{84.69 $\%$} & \multicolumn{1}{c}{\textcolor{red}{73.32} $\%$} & \multicolumn{1}{c}{52.32 $\%$} \\ 
\begin{tabular}{c} sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.84 $\%$}  & \multicolumn{1}{c}{58.42 $\%$} & \multicolumn{1}{c}{81.06 $\%$}& \multicolumn{1}{c}{49.11 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.69 $\%$} & \multicolumn{1}{c}{85.76 $\%$} & \multicolumn{1}{c}{75.34 $\%$} & \multicolumn{1}{c}{53.95 $\%$} \\ 
\begin{tabular}{c} sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.47 $\%$}  & \multicolumn{1}{c}{77.59 $\%$} & \multicolumn{1}{c}{81.50 $\%$} & \multicolumn{1}{c}{52.78 $\%$}\\ 
\begin{tabular}{c} Confidential sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.27 $\%$}  & \multicolumn{1}{c}{86.16 $\%$} & \multicolumn{1}{c}{76.94 $\%$} & \multicolumn{1}{c}{55.60 $\%$} \\ 
\begin{tabular}{c} sMCL (top 4)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.19 $\%$}  & \multicolumn{1}{c}{80.96 $\%$} & \multicolumn{1}{c}{80.72 $\%$} & \multicolumn{1}{c}{\textcolor{red}{54.55} $\%$} \\ 
\begin{tabular}{c} Confidential sMCL (top 4)  \end{tabular}& \begin{tabular}{c} \end{tabular}  & \multicolumn{1}{c}{98.24 $\%$}  & \multicolumn{1}{c}{85.87 $\%$} & \multicolumn{1}{c}{78.05 $\%$}& \multicolumn{1}{c}{55.79 $\%$}  \\  
\bottomrule
\end{tabular}
\end{center}
\caption{
Classification test set accuracy on CIFAR.
}\label{tbl:loc}
\end{table*}
\fi

\iffalse
\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{@{}lcccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Ensemble Size \end{tabular}}
 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} CIFAR-10 \end{tabular}} &  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} CIFAR-100 \end{tabular}} \\ 
& \multicolumn{1}{c}{} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} & \multicolumn{1}{c}{Oracle Accuracy}& \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} &\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}} 5 \end{tabular}} & \multicolumn{1}{c}{85.40} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{55.09 $\%$} \\
\begin{tabular}{c} sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{72.26 $\%$}& \multicolumn{1}{c}{42.31 $\%$} \\ 
\begin{tabular}{c} sMCL + Random (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{68.18 $\%$}& \multicolumn{1}{c}{51.72 $\%$} \\ 
\begin{tabular}{c} sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{73.44 $\%$}& \multicolumn{1}{c}{52.65 $\%$} \\ 
\begin{tabular}{c} sMCL + Random (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{95.11}  & \multicolumn{1}{c}{85.97} & \multicolumn{1}{c}{70.47 $\%$} & \multicolumn{1}{c}{53.21 $\%$} \\ 
\begin{tabular}{c} sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}& \multicolumn{1}{c}{} \\ 
\begin{tabular}{c} sMCL + Random (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{94.83}  & \multicolumn{1}{c}{85.78} & \multicolumn{1}{c}{71.69 $\%$} & \multicolumn{1}{c}{54.63 $\%$}\\ 
\begin{tabular}{c} sMCL (top 4)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ 
\begin{tabular}{c} sMCL + Random (top 4)  \end{tabular}& \begin{tabular}{c} \end{tabular}  & \multicolumn{1}{c}{94.61}  & \multicolumn{1}{c}{85.92} & \multicolumn{1}{c}{69.99 $\%$} & \multicolumn{1}{c}{55.35 $\%$} \\  
\midrule
\begin{tabular}{c} Independent \end{tabular} &\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}} 10 \end{tabular}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{85.47}& \multicolumn{1}{c}{92.43} & \multicolumn{1}{c}{55.98 $\%$} \\
\begin{tabular}{c} sMCL (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{79.31 $\%$} & \multicolumn{1}{c}{32.32 $\%$} \\ 
\begin{tabular}{c} sMCL + Random (top 1)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{78.13 $\%$} & \multicolumn{1}{c}{53.58 $\%$} \\ 
\begin{tabular}{c} sMCL (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{81.49 $\%$}& \multicolumn{1}{c}{49.35 $\%$} \\ 
\begin{tabular}{c} sMCL + Random (top 2)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.92} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{79.26 $\%$} & \multicolumn{1}{c}{55.31 $\%$} \\ 
\begin{tabular}{c} sMCL (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{81.61 $\%$} & \multicolumn{1}{c}{53.91 $\%$}\\ 
\begin{tabular}{c} sMCL + Random (top 3)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{98.88}  & \multicolumn{1}{c}{86.22} & \multicolumn{1}{c}{79.36 $\%$} & \multicolumn{1}{c}{56.16 $\%$} \\ 
\begin{tabular}{c} sMCL (top 4)  \end{tabular}& \begin{tabular}{c}\end{tabular}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{80.76 $\%$} & \multicolumn{1}{c}{55.11 $\%$} \\ 
\begin{tabular}{c} sMCL + Random (top 4)  \end{tabular}& \begin{tabular}{c} \end{tabular}  & \multicolumn{1}{c}{98.57}  & \multicolumn{1}{c}{86.33} & \multicolumn{1}{c}{79.11 $\%$}& \multicolumn{1}{c}{\bf 56.33 $\%$}  \\  
\bottomrule
\end{tabular}
\end{center}
\caption{
Results of the iterative attention-based inference scheme for
the object localization tasks.
We train convolutional
neural networks for bounding-box regression on the ILSVRC 2012 CLS-LOC dataset. locErr 
and mIoU mean
the top-1 localization error rate (\%)
and 
%Results of recursive attention-based inference applied simple regression network on ILSVRC CLS-LOC dataset. locErr: top-1 localization error rate (\%), mIOU: 
the mean of intersection over union of the prediction bounding-box and ground-truth,
respectively.
The performance improvements beyond the baseline inference without iterations
%DNN (due to fine-tuning DNN parameters under Simplified-SFNN) 
are calculated in the bracket.
}\label{tbl:loc}
\end{table*}
\fi
\iffalse
\begin{table}[]
\centering
\begin{tabular}{ccc}
\hline
\multicolumn{2}{c}{\multirow{2}{*}{Ensemble Method}}    & \multirow{2}{*}{Ensemble Accuracy} \\
\multicolumn{2}{c}{}                                    &                                    \\ \hline
\multicolumn{2}{c}{Independent}         & 81.29\%           \\ \hline
\multicolumn{2}{c}{Confidential sMCL}   & 80.04\%           \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{\extracolsep{\fill}}c@{}}Confidential sMCL\\ + Feature Sharing\end{tabular}}
    & $\lambda = 0.3$ & 83.37\%             \\
    & $\lambda = 0.5$ & 84.12\%             \\
    & $\lambda = 0.7$ & 84.22\%             \\
    & $\lambda = 0.9$ & 84.91\%             \\
    & $\lambda = 1.0$ & 84.52\%             \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{\extracolsep{\fill}}c@{}}Confidential sMCL\\ + Feature Sharing\\ + Overlap $K = 4$\end{tabular}}
    & $\lambda = 0.3$ & 84.99\%             \\
    & $\lambda = 0.5$ & 85.21\%             \\
    & $\lambda = 0.7$ & \bf{85.46\%}        \\
    & $\lambda = 0.9$ & 85.32\%             \\
    & $\lambda = 1.0$ & 85.24\%             \\ \hline
\end{tabular}
\caption{Improvement of ensemble gain from generalized features.}
\label{tbl:fs}
\end{table}
\fi

\iffalse
\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{@{}ccccllllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Ensemble Method \end{tabular}} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Overlap Parameter $K$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=5$ \end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} Ensemble Size $M=10$ \end{tabular}} \\ &
                                \multicolumn{1}{c}{} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} &
                                \multicolumn{1}{c}{Oracle Accuracy} &
                                \multicolumn{1}{c}{Ensemble Accuracy} \\ \midrule
\begin{tabular}{c} Independent \end{tabular} & &
    \multicolumn{1}{c}{86.58 $\%$} &
    \multicolumn{1}{c}{81.29 $\%$} &
    \multicolumn{1}{c}{88.11 $\%$} &
    \multicolumn{1}{c}{81.27 $\%$} \\ \midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 1 \end{tabular}} &
    \multicolumn{1}{c}{93.84 $\%$} &
    \multicolumn{1}{c}{38.67 $\%$} &
    \multicolumn{1}{c}{100.0 $\%$} &
    \multicolumn{1}{c}{25.47 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{95.16 $\%$} &
    \multicolumn{1}{c}{79.65 $\%$} &
    \multicolumn{1}{c}{97.34 $\%$} &
    \multicolumn{1}{c}{77.86 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{95.92 $\%$} &
    \multicolumn{1}{c}{83.75 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 2 \end{tabular}} &
    \multicolumn{1}{c}{94.79 $\%$} &
    \multicolumn{1}{c}{72.19 $\%$} &
    \multicolumn{1}{c}{96.95 $\%$}&
    \multicolumn{1}{c}{49.68 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{95.37 $\%$} &
    \multicolumn{1}{c}{81.47 $\%$} &
    \multicolumn{1}{c}{98.41 $\%$} &
    \multicolumn{1}{c}{79.88 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{95.84 $\%$} &
    \multicolumn{1}{c}{84.40 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 3 \end{tabular}} &
    \multicolumn{1}{c}{91.57 $\%$}  &
    \multicolumn{1}{c}{79.08 $\%$} &
    \multicolumn{1}{c}{98.13 $\%$}&
    \multicolumn{1}{c}{72.05 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{93.69 $\%$} &
    \multicolumn{1}{c}{82.55 $\%$} &
    \multicolumn{1}{c}{98.23 $\%$} &
    \multicolumn{1}{c}{81.46 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{94.13 $\%$} &
    \multicolumn{1}{c}{84.37 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\\midrule
    
\begin{tabular}{c} sMCL
\end{tabular} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 4 \end{tabular}} &
    \multicolumn{1}{c}{92.00 $\%$}  &
    \multicolumn{1}{c}{80.56 $\%$} &
    \multicolumn{1}{c}{96.49 $\%$}&
    \multicolumn{1}{c}{75.76 $\%$}  \\ 
\begin{tabular}{c} Confidential sMCL
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{97.66 $\%$} &
    \multicolumn{1}{c}{82.02 $\%$} &
    \multicolumn{1}{c}{92.05 $\%$} &
    \multicolumn{1}{c}{82.57 $\%$} \\ 
\begin{tabular}{c} Confidential sMCL \\+ Feature Sharing
\end{tabular}&\begin{tabular}{c}\end{tabular}&
    \multicolumn{1}{c}{93.44 $\%$} &
    \multicolumn{1}{c}{84.46 $\%$}  &
    \multicolumn{1}{c}{ $\%$}&
    \multicolumn{1}{c}{ $\%$} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Classification test set accuracy on CIFAR-10 using entropy.
}\label{tbl:loc}
\end{table*}
\fi

==> exp_backup.tex <==
\section{Experiments}
\label{sec:exp}

We evaluate our algorithm for both classification and foreground-background segmentation tasks using CIFAR-10 \cite{cifar09}, SVHN \cite{11SVHN} and iCoseg \cite{icoseg10} datasets.
%on CIFAR-10 \cite{cifar09}, SVHN \cite{11SVHN} and iCoseg \cite{icoseg10} datasets, respectively.
In all experiments, we compare the performance of CMCL with those of traditional IE and MCL using deep models. % for comparison.
We leave the detail of the setup including model architectures in the supplementary material.
\textcolor{blue}{Our code is available at \url{https://github.com/chhwang/cmcl}.}

\subsection{Image Classification} \label{ssec:exp-cls}
%We report experimental results for image classification task on CIFAR-10 dataset \cite{cifar09}.
\noindent {\bf Setup.}
The CIFAR-10 dataset consists of 50,000 training and 10,000 test images with 10 image classes where each image consists of $32\times32$ RGB pixels.
The SVHN dataset consists of 73,257 training
and 26,032 test images.\footnote{We do not use the extra SVHN dataset for training.}
We pre-process the images with global contrast normalization and ZCA whitening 
following \cite{maxout,wrn16}, and do not use any data augmentation.
Using these datasets, we train various CNNs, e.g., VGGNet \cite{vggnet}, GoogLeNet \cite{googlenet}, and ResNet \cite{resnet}.
Similar to \citep{wrn16}, we use the softmax classifier, and train each model by minimizing the cross-entropy loss using the stochastic gradient descent method with Nesterov momentum.

%metric
For evaluation, we measure the top-1 and oracle error rates on the test dataset.
The top-1 error rate is calculated by averaging output probabilities from all models \textcolor{blue}{and predicting the class from the largest averaged probability}.
%This metric presents the practical performance of ensemble.
The oracle error rate is the rate of classification failure over all outputs of individual ensemble members for a given input, i.e., if none of the
members predict the correct class for an input.
Note that this metric measures the level of specialization and diversity of ensemble members. While a lower oracle error rate suggests higher diversity, a lower oracle error rate does not always bring a higher top-1 accuracy as this metric does not reveal the level of overconfidence of each model.
%For example, 10 ensemble models classifying 10 classes can always achieve 0\% oracle error rate by making each model to return the same prediction for all input data, which is different from others' predictions.
By collectively measuring the top-1 and oracle error rates, one can grasp the level of specialization and confidence of a model.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Ensemble\\Method\end{tabular}&\begin{tabular}[c]{@{}c@{}}Feature\\ Sharing\end{tabular}
&\begin{tabular}[c]{@{}c@{}}Stochastic\\ Labeling\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Oracle\\ Error Rate\end{tabular}&
\begin{tabular}[c]{@{}c@{}}Top-1\\ Error Rate\end{tabular} \\ \hline
IE    & -            & -           & 10.65\%       & 15.34\%       \\ \hline
MCL   & -            & -           & 4.40\%        & 60.40\%       \\ \hline
\multirow{3}{*}{CMCL}
            & -              & -             & 4.49\%        & 15.65\%       \\
            & \checkmark     & -             & 5.12\%        & 14.83\%       \\
            & \checkmark     & \checkmark    & \bf{3.32\%}   & \bf{14.78\%}  \\ \hline
\end{tabular}}
\caption{Classification test set error rates on CIFAR-10 using various ensemble methods.
}
\label{tbl:comparison}
\end{table}

\noindent {\bf Contribution by each technique.} 
\textcolor{blue}{Table \ref{tbl:comparison} validates our suggested methods by comparing against legacy ensemble methods. We evaluate an ensemble of five simple CNN models where each model has two convolutional layers followed by a fully-connected layer. 
We incrementally apply our optimizations to gauge the stepwise improvement by each component. One can note that CMCL significantly outperforms MCL in the top-1 error rate even without feature sharing or stochastic labeling while it presents a comparable oracle error rate.
%with the one of MCL.
With feature sharing over confident oracle loss, the top-1 error rates are improved compared to those that employ only confident oracle loss.
Applying stochastic labeling on top of feature sharing further also improves the top-1 error rate. 
This indicates that stochastic labeling not only reduces a computation but also produces similar regularization effect as feature sharing.}


\begin{table*}[t]
\centering
\begin{tabular}{ccllll}
\hline
\multirow{2}{*}{Ensemble Method}   & \multirow{2}{*}{$K$} & \multicolumn{2}{l}{\hspace{12mm}Ensemble Size $M=5$}  & \multicolumn{2}{l}{\hspace{11mm}Ensemble Size $M=10$}     \\
                                   &                    & Oracle Error Rate & Top-1 Error Rate    & Oracle Error Rate & Top-1 Error Rate    \\ \hline
IE  & -  & \hspace{7mm}10.65\%                   & \hspace{6mm}15.34\%                    & \hspace{6mm}9.26\%                  & \hspace{6mm}15.34\%           \\ \hline
\multirow{4}{*}{MCL} 
             & 1  & \hspace{8mm}4.40\%                    & \hspace{6mm}60.40\%                    & \hspace{6mm}\textbf{0.00\%}    & \hspace{6mm}76.88\%            \\
             & 2 & \hspace{8mm}3.75\%                    & \hspace{6mm}20.66\%                    & \hspace{6mm}1.46\%                   & \hspace{6mm}49.31\%                    \\
             & 3 & \hspace{8mm}4.73\%                    & \hspace{6mm}16.24\%                    & \hspace{6mm}1.52\%                 & \hspace{6mm}22.63\%                    \\
             & 4 & \hspace{8mm}5.83\%                    & \hspace{6mm}15.65\%                    & \hspace{6mm}1.82\%                   & \hspace{6mm}17.61\%                    \\ \hline
\multirow{4}{*}{CMCL}
            &  1 & \hspace{8mm}\textbf{3.32\%}          & \hspace{6mm}14.78\%           & \hspace{6mm}1.96\%                   & \hspace{6mm}14.28\%                    \\
            &  2 & \hspace{8mm}3.69\% & \hspace{6mm}\textbf{14.25\% (-7.11\%)}          & \hspace{6mm}1.22\%                   & \hspace{6mm}13.95\%                   \\
            &  3 & \hspace{8mm}4.38\%                    & \hspace{6mm}14.38\%           & \hspace{6mm}1.53\%                   & \hspace{6mm}14.00\%                    \\
            &  4 & \hspace{8mm}5.82\%                    & \hspace{6mm}14.49\%           & \hspace{6mm}1.73\%                  & \hspace{6mm}\textbf{13.94\% (-9.13\%)} \\ \hline
\end{tabular}
\caption{
Classification test set error rates on CIFAR-10 with varying values of the overlap parameter $K$ explained in \ref{ssec:exp-cls}. 
We use CMCL with both feature sharing and stochastic labeling.
Boldface values in parentheses represent the relative reductions from the best results of MCL and IE.
}\label{tbl:cifar10}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{cccllll}
\hline
\multirow{2}{*}{Model Name}               &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ensemble\\Method\end{tabular}} &
\multicolumn{2}{l}{\hspace{18mm}CIFAR-10} &
\multicolumn{2}{l}{\hspace{22mm}SVHN} \\
& &
Oracle Error Rate  &
Top-1 Error Rate &
Oracle Error Rate  &
Top-1 Error Rate   \\ \hline
\multirow{4}{*}{VGGNet-17}    & - (single)           & \hspace{0mm}10.65\%                    &\hspace{6mm}10.65\%    & \hspace{8mm}5.22\%                    & \hspace{7mm}5.22\%       \\
& IE           & \hspace{0mm}3.27\%                    & \hspace{7mm}8.21\%    & \hspace{8mm}1.99\%                    & \hspace{7mm}4.10\%       \\
                           & MCL          & \hspace{0mm}\textbf{2.52\%}                    & \hspace{6mm}45.58\%    & \hspace{8mm}\textbf{1.45\%}                    & \hspace{6mm}45.30\%         \\
                           & CMCL         & \hspace{0mm}2.95\% & \hspace{7mm}\textbf{7.83\% (-4.63\%)}  & \hspace{8mm}1.65\% & \hspace{7mm}\textbf{3.92\% (-4.39\%)} \\ \hline
\multirow{4}{*}{GoogLeNet-18} & - (single)           & \hspace{0mm}10.15\%                    & \hspace{6mm}10.15\%    & \hspace{8mm}4.59\%                    & \hspace{7mm}4.59\%       \\
& IE           & \hspace{0mm}3.37\%                    & \hspace{7mm}7.97\%    & \hspace{8mm}1.78\%                    & \hspace{7mm}3.60\%       \\
                           & MCL          & \hspace{0mm}\textbf{2.41\%}           & \hspace{6mm}52.03\% & \hspace{8mm}1.39\%           & \hspace{6mm}37.92\%         \\
                           & CMCL         & \hspace{0mm}2.54\%                    & \hspace{7mm}\textbf{7.44\% (-6.65\%)}
                           &\hspace{8mm}\textbf{1.31\%}                    & \hspace{7mm}\textbf{3.46\% (-3.89\%)}  \\ \hline
\multirow{4}{*}{ResNet-32} & - (single)           & 12.89\%                    & \hspace{6mm}12.89\%    & \hspace{8mm}5.05\%                    & \hspace{7mm}5.05\%       \\
& IE           & \hspace{0mm}3.54\%                    & \hspace{7mm}9.50\% & \hspace{8mm}1.81\%                    & \hspace{7mm}3.84\%         \\
                           & MCL          & \hspace{0mm}3.11\%           & \hspace{6mm}53.74\% & \hspace{8mm}1.69\%           & \hspace{6mm}39.76\%         \\
                           & CMCL         & \hspace{0mm}\textbf{2.89\%}                    & \hspace{7mm}\textbf{8.42\% (-11.37\%)}
                           & \hspace{8mm}\textbf{1.41\%}                    & \hspace{7mm}\textbf{3.56\% (-7.29\%)}\\ \hline
\end{tabular}
\caption{Classification test set error rates on CIFAR-10 and SVHN for various large-scale CNN models. 
\textcolor{blue}{We train an ensemble of 5 models, and use CMCL with both feature sharing and stochastic labeling.}
Boldface values in parentheses indicate relative error rate reductions from the best results of MCL and IE.}
\label{tbl:deep}
\end{table*}


%As the final step of our improvements, 
\noindent {\bf Overlapping.}
To address the overconfidence issue, we now consider picking $K$ specialized models instead of having only one specialized model, similar to the techniques applied for original MCL~\citep{mcl12,mcl16}. This is easily achieved by modifying the constraint \eqref{eq:const} as $\sum_{m=1}^M v_i^m = K$, where $K$ is an overlap parameter that controls training data overlap between the models. This simple but natural scheme brings extra gain in top-1 performance by generalizing each model better as reported by the authors.
Table~\ref{tbl:cifar10} compares the performance of various ensemble methods with varying values of $K$.
%We found that CMCL achieves its best performance when $K$ is given as more than one.
\textcolor{blue}{
Under the choice of $K=4$, CMCL of 10 CNNs provides 9.13\% relative reduction in the top-1 error rates from the corresponding IE.
We remark that IE has similar error rates on both 5 and 10 CNNs, which implies that the performance of CMCL might not be impossible via IE even if one increases the number of models in IE.}



\noindent {\bf Large-scale CNNs.} 
We now evaluate the performance of our ensemble method when it is applied to larger-scale CNN models for image classification tasks on CIFAR-10 and SVHN datasets.
%To show model independent properties of our methods, we choose various representative designs of CNN: 
Specifically, we test VGGNet~\cite{vggnet}, GoogLeNet~\cite{googlenet}, and ResNet~\cite{resnet}. %In these %models, it would be non-trivial to determine features of which %layer should be shared for the best performance. 
We share the non-linear activated features right before the first pooling layer as stated in Section \ref{sec:feature-sharing}, i.e. the 11-th ReLU activation for ResNet with 32 layers and the second ReLU activation for VGGNet with 17 layers or GoogLeNet with 18 layers. %\textcolor{red}{
By doing this, we expect to maximize the regularization effect of feature sharing while minimizing the statistical dependencies among the ensemble models. % as low as possible.
For all models, we choose the best hyper-parameters for confident oracle loss among the penalty parameter $\beta \in \{0.5,0.75,1,1.25,1.5\}$ and the overlapping parameter $K\in\{2,3,4\}$. 
Table~\ref{tbl:deep} shows that CMCL consistently outperforms all baselines with respect to the top-1 error rate while producing comparable oracle error rates to those of MCL.
\textcolor{blue}{We also evaluate the performance by applying the feature sharing to IE as shown in Figure \ref{fig5:c}.
Even though the feature sharing also improves the performance of IE, CMCL still outperforms IE with respect to the top-1 error rate.
In particular, our method provides 5.77\% relative reduction from the IE with feature sharing under the choice of $M=10$. We also remark that IE with feature sharing has similar error rates as the ensemble size increases, while CMCL does not (i.e., the gain is more significant for CMCL).}




\begin{figure*}[t]
\includegraphics[width=\textwidth]{figures/iCoseg_final_ver1.pdf}
\caption{Prediction results of foreground-background segmentation for a few sample images. 
A test error rate is shown below each prediction.
The ensemble models trained by CMCL and MCL generate high-quality predictions specialized for certain images.
%, and red rectangles indicate the most accurate segmentation (i.e., lowest error rate). 
%
}\label{fig:icoseg}
\end{figure*}

\begin{figure*} [h] \centering
\subfigure[]
{\epsfig{file=figures/Resnet_Top_1_error.eps, width=0.32\textwidth}\label{fig5:c}}
%performance.eps
\,
\subfigure[]
{\epsfig{file=figures/top1_iCoseg_final.eps, width=0.32\textwidth}\label{fig5:a}}
\,
\subfigure[]
{\epsfig{file=figures/oracle_icoseg_final.eps, width=0.32\textwidth}\label{fig5:b}}
%\,
%\subfigure[Test set accuracy comparison for varying the ensemble size $M$.]
%{\epsfig{file=figures/ensemble_acc.eps, width=0.31\textwidth}\label{fig2:c}}
\caption{(a) Classification test set error rates on CIFAR-10. We measure the top-1 error rate on CIFAR-10 using an ensemble of $M$ ResNets with 32 layers. (b) Top-1 error rate and (c) oracle error rate on iCoseg
by varying the ensemble sizes. 
%The ensemble models trained by CMCL consistently improves the top-1 error rate over baselines.
}\label{fig:icosef}
\end{figure*}

\subsection{Foreground-Background Segmentation}
\label{ssec:exp-icoseg}

In this section, we evaluate if ensemble models trained with CMCL produce high-quality segmentation of foreground and background of an image with the iCoseg dataset.
The foreground-background segmentation is formulated as a pixel-level classification problem with 2 classes, i.e., 0 (background) or 1 (foreground). To tackle the problem, we design fully convolutional networks (FCNs) model~\cite{long2015fully} based on the decoder architecture presented in \citep{radford2015unsupervised}.
The dataset consists of 38 groups of related images with pixel-level ground truth on foreground-background segmentation of each image. We only use images that are larger than $300 \times 500$ pixels.
For each class, we randomly split $80\%$ and $20\%$ of the data into training and test sets, respectively. We train on $75 \times 125$ resized images using the bicubic interpolation~\cite{keys1981cubic}. 
%We train an ensemble of two FCNs for 200 epochs in total.
Similar to \cite{mcl12,mcl16}, we initialize the parameters of FCNs with those trained by IE for MCL and CMCL.
\textcolor{blue}{For all experiments, CMCL is used with both feature sharing and stochastic labeling.}
We leave the detail of the setup including model architectures in the supplementary material.

%metric
Similar to \cite{mcl12}, we define the percentage of incorrectly labeled pixels as prediction error rate.
We measure the oracle error rate (i.e., the lowest error rate over all models for a given input) and the top-1 error rate.
The top-1 error rate is measured by following the predictions of the member model that has a lower pixel-wise entropy, i.e., picking the output of a more confident model.
For each ensemble method, we vary the number of ensemble models and measure the oracle error rate and test error rate.
Figure~\ref{fig:icosef} shows both oracle and top-1 error rates for all ensemble methods. We remark that the ensemble models trained by CMCL consistently improves the top-1 error rate over baselines. In an ensemble of 5 models, we find that CMCL achieve up to $6.77\%$ relative reduction in the top-1 error rate from the corresponding IE.
%(see Table \ref{Tab:icoseg}).
%This implies that training the uncertainty \ks{not only improves the confidence of each model but also makes them  more specialized.}
As shown in Figure \ref{fig:icoseg}, an individual model trained by CMCL generates high-quality solutions by specializing itself in specific images (e.g., model 1 is specialized for `duck' while model 2 is specialized for `lobster') while each model trained by IE does not. 




